Rethinking Certification for Trustworthy Machine Learning-Based Applications

Machine Learning (ML) is increasingly used to implement advanced applications with non-deterministic behavior, which operate on the cloud-edge continuum. The pervasive adoption of ML is urgently calling for assurance solutions assessing applications non-functional properties (e.g., fairness, robustness, privacy) with the aim to improve their trustworthiness. Certification has been clearly identified by policymakers, regulators, and industrial stakeholders as the preferred assurance technique to address this pressing need. Unfortunately, existing certification schemes are not immediately applicable to non-deterministic applications built on ML models. This article analyzes the challenges and deficiencies of current certification schemes, discusses open research issues, and proposes a first certification scheme for ML-based applications.

==> other/02_cert_overview.tex <==
\tikzset{
    entity/.style={
      draw,
      ellipse,
      very thin
    },
    artifact/.style={
      rectangle,
      draw,
      rounded corners,
      %fill=VeryLightGrey!50
    },
    service/.style={
      chamfered rectangle,
      chamfered rectangle angle=30,
      draw,
      %fill=VeryLightGrey!120
    },
    every node/.style={
        font={\scriptsize},
        text centered,
    },
    on link/.style={
      fill=white,
    },   
    connector/.style={
        >=stealth,
    },
    connector assurance/.style={
        >=Stealth,
        dashed
    },
    on slide/.code args={<#1>#2}{%
      \only<#1>{\pgfkeysalso{#2}}%
    },
    highlight base/.style={
      very thick
    },
    highlight/.style={
      highlight base,
      fill=LightGoldenRod,
    },
    highlight profile/.style={
      \highlightprofilecolor
    },
    highlight double/.style={
      double=LightGoldenRod
    },
    highlight text/.style={
      text=Goldenrod,
    },
    highlight link/.style={
      %thick,
      color=Goldenrod
    },
    highlight light/.style={
      fill=LightGoldenRod!20
    },
      element/.style={
          inner sep=1.5pt,
          font=\footnotesize
      },
      connector/.style={
          >=Stealth,
      },
      lattice layer label/.style={
          text width=2.9cm,
          font={\footnotesize},
      },
      not chosen color/.style={
          black!50
      },
      lattice layer separator/.style={
          dashed,
      },
      service label/.style={
          fill=white,
          circle,
          draw,
          very thick,
          inner sep=2.5pt,
      },
      lattice element bound/.style={
          fill=black!15,
          double
      },
      lattice element selected/.style={
          fill=Goldenrod!15,
          double
      },
      lattice element not chosen/.style={
          not chosen color,
          densely dotted
      },
      lattice element not chosen link/.style={
          not chosen color,
          densely dotted
      },
      service element not chosen/.style={
          text=black!50,
          draw=black!50,
          dashed,
      },
      header/.style={
      },
      main box/.style={
          font={\small}
      },
      link/.style={
        >=Latex,
      },
      activity/.style={
        fill=white
      },
}


\begin{tikzpicture}


    \node[entity] (ca) at (-1.5, 0) {CA};

    \node[artifact] (cm) at (-1.5, -1.65) {\makecell{Certification\\Model \mathct}};

    \draw[->, link] (ca) to node[on link]{prepares} (cm);

    \node[artifact] (properties) at (2.35, -1.65) (property)  {\makecell{Property \mathproperty}};

    \node[service] (target) at (2.35, -3.2) {\makecell{Target \mathtarget}};

    \draw[->, link] (cm) to node[on link] {evaluates} (property);

    %\draw[->, link] (cm) to node[on link] {to assess} (target);
    \draw[->, link] (property) to node[on link] {on} (target);

    \node[artifact] (evidence collection model) at (cm |- target) {\makecell{Evidence\\Coll. Model \mathevidcollection}};

    \node[entity, inner sep=1pt] (lab) at ([yshift=-40]evidence collection model.south) {\makecell{Accredited\\Lab}};

    \draw[->, link] (target) to node[on link] {according to} (evidence collection model);

    %\node[entity, inner sep=1pt] (lab) at (cm |- target)  {\makecell{Accredited\\Lab}}; %(-1.5, -3.65) {\makecell{Accredited\\Lab}};

    \draw[->, link] (evidence collection model) to node[on link]{executed by} (lab);

    \draw[->, link] (lab) to node[on link] (against) {against} (target);

    \node[artifact] at ([yshift=-35]against.south) (evidence) {Evidence};

    \draw[->, link] (against) to node[on link] {collecting} (evidence);

    \node[artifact] at ([yshift=-35]evidence.south) (certificate) {\makecell{Certificate}};

    \draw[ link, ->] (evidence) to node[on link]{on success} (certificate);

    %\draw[link, ->, bend right=70] (certificate.east) to node[xshift=20, near end, on link] (includes) {includes} (evidence.east);

    %\draw[->, link, bend right=45] (includes) to (target.east);

    %\draw[->, link, bend right=55] (includes.east) to (property.east);


\end{tikzpicture}

==> other/05_summary_table.tex <==
\begin{table*}[!ht]
    \caption{Summary of the certification scheme applied on our scenario.}\label{tbl:exp-summary}
    \begin{adjustbox}{max totalsize={\textwidth}{\textheight},center}
        \begin{tabular}{l p{.39\textwidth} p{.13\linewidth} p{.4\textwidth} c}
            \toprule
            $f$ & \mathproperty & \mathtarget & \mathevidcollection & Outcome\\
            \midrule
            \\
            \factorData &
            \begin{minipage}[t]{\linewidth}
                Robustness against inference\-/time attacks\\
                (Absence of adversarial poisoning in the training set)
            \end{minipage} &
            Training set & 
            \begin{minipage}{\linewidth}
                $-$ Check the presence of poisoned samples\\
                $-$ \emph{evidence}: poisoned samples$=$$\emptyset$
            \end{minipage}&
            %Awarded
            \ok
            \\
            \\
            \factorProcess &
            \begin{minipage}{\linewidth}
                Robustness against inference\-/time attacks\\
                (Usage of randomized smoothing and adversarial training)
            \end{minipage}&
            Training process &
            \begin{minipage}{\linewidth}
                $-$ Check the training process and checkpoints\\
                $-$ \emph{evidence}: training process does not include \emph{randomized smoothing} and \emph{adversarial training}
            \end{minipage}&
            %Not awarded
            \notok
            \\
            \\
            \factorModel &
            \begin{minipage}[t]{\linewidth}
                Robustness against inference\-/time attacks\\
                (Ineffectiveness of adversarial attacks)
            \end{minipage}&
                Malware detector (Deep Learning model)&
            \begin{minipage}[t]{\linewidth}
                $-$ Craft and send adversarial samples to the ML model \\ %service's sidecar\\
                $-$ \emph{evidence}: recall$=$0 %$\vert$recall$\vert$$=$0.96
            \end{minipage}&
            %Awarded
            \notok\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

